Ziya2: Data-centric Learning is All LLMs Need

Various large language models (LLMs) have been proposed in recent years, including closed- and open-source ones, continually setting new records on multiple benchmarks. However, the development of LLMs still faces several issues, such as high cost of training models from scratch, and continual pre-training leading to catastrophic forgetting, etc. Although many such issues are addressed along the line of research on LLMs, an important yet practical limitation is that many studies overly pursue enlarging model sizes without comprehensively analyzing and optimizing the use of pre-training data in their learning process, as well as appropriate organization and leveraging of such data in training LLMs under cost-effective settings. In this work, we propose Ziya2, a model with 13 billion parameters adopting LLaMA2 as the foundation model, and further pre-trained on 700 billion tokens, where we focus on pre-training techniques and use data-centric optimization to enhance the learning process of Ziya2 on different stages. We define three data attributes and firstly establish data-centric scaling laws to illustrate how different data impacts LLMs. Experiments show that Ziya2 significantly outperforms other models in multiple benchmarks especially with promising results compared to representative open-source ones. Ziya2 (Base) is released at https://huggingface.co/IDEA-CCNL/Ziya2-13B-Base and https://modelscope.cn/models/Fengshenbang/Ziya2-13B-Base/summary.

==> abs.tex <==
Various large language models (LLMs) have been proposed in recent years, including closed- and open-source ones, continually setting new records on multiple benchmarks. However, the development of LLMs still faces several issues, such as high cost of training models from scratch, and continual pre-training leading to catastrophic forgetting, etc. Although many such issues are addressed along the line of research on LLMs, an important yet practical limitation is that many studies overly pursue enlarging model sizes without comprehensively analyzing and optimizing the use of pre-training data in their learning process, as well as appropriate organization and leveraging of such data in training LLMs under cost-effective settings. In this work, we propose Ziya2, a model with 13 billion parameters adopting LLaMA2 as the foundation model, and further pre-trained on 700 billion tokens, where we focus on pre-training techniques and use data-centric optimization to enhance the learning process of Ziya2 on different stages. Experiments show that Ziya2 significantly outperforms other models in multiple benchmarks especially with promising results compared to representative open-source ones. Ziya2 (Base) is released at https://huggingface.co/IDEA-CCNL/Ziya2-13B-Base and https://modelscope.cn/models/Fengshenbang/Ziya2-13B-Base/summary.

==> notes/notes-1104.tex <==

1. 什么样的训练数据对模型效果的影响
2. 数据centric的LLM训练

------

11. 另外一个很大的问题就是整个文章里面的时态不统一，统一成现在时

12. 然后就是全文你们俩再过一遍，最后元贺在此基础上再过一遍，不论改了还是没改的地方，只要不是我看过的，都要把文字写作看一遍，每段最后一行不要出现一个词或者半个词，也不要等我来说改哪里，全部都要看一下。方法这里可能没有时间细看了，但是粗一看问题不少，还有打错的词


17. 3.3结果要写出来ziya2的巨大优势
18. fig1变大一点，两边的框定格

---------
所有的
1. figure 6 不同的阶段用不同的底色，底色跟前面图的颜色的对应上1. 这个试了，跟线和节点的颜色会冲突,先不加
2. 例子都改成斜体
3. figure 4 字变大，
4. Section 2 蓝色：approach这里这句话，要说一下数据在这个过程里怎么加强的。或者在这句后面加一句也行
5. 2.3加Roadmap，简单说后面的内容结构就行
6. evaluation 加入 Roadmap
7. 3.3和3.4的内容要重新整理一下；3.4要有个类似帽子的东西盖住下面三个阶段的解读
8. conclusion 重写
9. 2.1最开始的红色，这句话放到其他地方去，或者搞个脚注放在什么位置
10. 2.1红色全部重写。这里红色地方全部要重写，基本上没把事情说清楚，还有文字也不行。一直在跟你强调data factory，你在很多地方就不要再说pipeline了，不要把自己的工作搞low了，都按照一个系统化的数据工厂的角度来写
11. 另外一个很大的问题就是整个文章里面的时态不统一，现在，过去甚至将来时都有，你们把所有我还没动过的地方的时态都统一成现在时
12. 然后就是全文你们俩再过一遍，最后元贺在此基础上再过一遍，不论改了还是没改的地方，只要不是我看过的，都要把文字写作看一遍，每段最后一行不要出现一个词或者半个词，也不要等我来说改哪里，全部都要看一下。方法这里可能没有时间细看了，但是粗一看问题不少，还有打错的词
13. appendix 的图 最后这种颜色可以用浅蓝色
15. strategy进行修改
16. figure2 修改完成
17. 3.3结果要写出来ziya2的巨大优势
18. fig1变大一点，两边的框定格
19. figure3引用
20. figure1 文字对应上
21. intro增加3阶段数据描述
22. 表1调整了指标和顺序

